Quantified Linear and Polynomial Arithmetic Satisfiability via Template-based Skolemization

The problem of checking satisfiability of linear real arithmetic (LRA) and non-linear real arithmetic (NRA) formulas has broad applications, in particular, they are at the heart of logic-related applications such as logic for artificial intelligence, program analysis, etc. While there has been much work on checking satisfiability of unquantified LRA and NRA formulas, the problem of checking satisfiability of quantified LRA and NRA formulas remains a significant challenge. The main bottleneck in the existing methods is a computationally expensive quantifier elimination step. In this work, we propose a novel method for efficient quantifier elimination in quantified LRA and NRA formulas. We propose a template-based Skolemization approach, where we automatically synthesize linear/polynomial Skolem functions in order to eliminate quantifiers in the formula. The key technical ingredients in our approach are Positivstellens\"atze theorems from algebraic geometry, which allow for an efficient manipulation of polynomial inequalities. Our method offers a range of appealing theoretical properties combined with a strong practical performance. On the theory side, our method is sound, semi-complete, and runs in subexponential time and polynomial space, as opposed to existing sound and complete quantifier elimination methods that run in doubly-exponential time and at least exponential space. On the practical side, our experiments show superior performance compared to state-of-the-art SMT solvers in terms of the number of solved instances and runtime, both on LRA and on NRA benchmarks.

==> checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced - yes
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results - yes
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper - yes
\end{itemize}

Does this paper make theoretical contributions? - yes
\begin{itemize}
	\item All assumptions and restrictions are stated clearly and formally - yes
	\item All novel claims are stated formally (e.g., in theorem statements) - yes
	\item Proofs of all novel claims are included - yes
	\item Proof sketches or intuitions are given for complex and/or novel results - yes
	\item Appropriate citations to theoretical tools used are given - yes
	\item All theoretical claims are demonstrated empirically to hold - yes
	\item All experimental code used to eliminate or disprove claims is included - yes
\end{itemize}

Does this paper rely on one or more datasets? - yes
\begin{itemize}
	\item A motivation is given for why the experiments are conducted on the selected datasets - yes
	\item All novel datasets introduced in this paper are included in a data appendix - yes
	\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes - yes
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations - yes
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available - yes
	\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing - yes
\end{itemize}

Does this paper include computational experiments? - yes
\begin{itemize}
	\item Any code required for pre-processing data is included in the appendix - yes
	\item All source code required for conducting and analyzing the experiments is included in a code appendix - yes
	\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes - yes
	\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from - yes
	\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results - yes
	\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks - yes
	\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics - yes
	\item This paper states the number of algorithm runs used to compute each reported result - yes
	\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information - yes
	\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank) - yes
	\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments - yes
	\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting - yes
	
\end{itemize}



==> geometry.tex <==
\section{Tools from Algebraic Geometry}

In this section, we define the problem of {\em satisfiability of polynomial entailment} and formally introduce the theorems used in our algorithm.

Let $V = \{x_1, \ldots, x_r\}$ be a set of real-valued variables, $\Phi = \{p_0 \bowtie 0, \dots, p_m \bowtie 0\}$ a set of polynomial inequalities over $V$, and $\psi = (p \bowtie 0)$ a polynomial inequality over $V$, where each  $\bowtie \in \{\ge, >\}$.

The {\em satisfiability of polynomial entailment} problem asks for necessary and sufficient conditions for satisfiability of the following formula:  

\begin{equation} \label{eq:ent}
	\forall x_1.\dots\forall x_r.\,\, (\Phi \Longrightarrow \psi)
\end{equation}
This problem has been studied extensively in Real algebraic geometry and the following theorems provide a reduction from this problem to solving a system of polynomial inequalities, for which sub-exponential algorithms exist~\cite{grigor1988solving}. In particular, our algorithm will utilize the following results:

\begin{theorem}[{Farkas' Lemma \cite{farkas1902theorie}}]%{theorem}{Farkas}
	\label{thm:Farkas'}
	\index{Farkas' lemma}
	Consider a set $V = \{x_1, \ldots, x_r\}$ of real-valued variables and the following system $\Phi$ of equations over $V$:
	\begin{equation*}
		\Phi := 
		\begin{cases}
			a_{1,0} + a_{1,1} \cdot x_1 + \ldots + a_{1,r} \cdot x_r \ge 0\\
			\hfil \vdots\\
			a_{m,0} + a_{m,1} \cdot x_1 + \ldots + a_{m,r} \cdot x_r \ge 0\\
		\end{cases}.
	\end{equation*}
	When $\Phi$ is satisfiable, it entails a linear inequality $$\psi := c_0 + c_1 \cdot x_1 + \dots + c_r \cdot x_r \ge 0$$
	if and only if $\psi$ can be written as non-negative linear combination of the inequalities in $\Phi$ and the trivial inequality $1 \ge 0,$ i.e.~if there exist non-negative real numbers $y_0,\dots,y_m$ such that 
	$$
	\begin{matrix}
		c_0 = y_0 + \sum_{i=1}^k y_i \cdot a_{i, 0};\\
		c_1 = \sum_{i=1}^k y_i \cdot a_{i, 1};\\
		\vdots\\
		c_r = \sum_{i=1}^k y_i \cdot a_{i, r}.
	\end{matrix}
	$$
	%Moreover, $\Phi$ is unsatisfiable if and only if $-1 \ge 0$ can be derived as above. \
\end{theorem}

Farkas' Lemma provides a sound and complete method when both $\Phi$ and $\phi$ in (\ref{eq:ent}) are linear. In such cases, we introduce fresh real valued variables $y_1, \dots y_r$ and convert (\ref{eq:ent}) into the following fully existentially quantified formula:

\[
\exists y_1 \dots \exists y_r. \bigwedge y_i \geq 0 \wedge \begin{pmatrix}
	c_0 = y_0 + \sum_{i=1}^k y_i \cdot a_{i, 0};\\
	c_1 = \sum_{i=1}^k y_i \cdot a_{i, 1};\\
	\vdots\\
	c_r = \sum_{i=1}^k y_i \cdot a_{i, r}.
\end{pmatrix}
\]
The above formula is then equivalent to (\ref{eq:ent}) due to Farkas' Lemma (Theorem \ref{thm:Farkas'}). 

The following result considers the case where $\Phi$ is restricted to be linear and $\phi$ is a polynomial of arbitrary degree:

\begin{theorem}[{Handelman's Theorem \cite{handelman1988representing}}]%{theorem}{Handelman}
	\label{thm:handel}
	\index{Handelman's theorem}
	Consider a set $V = \{x_1, \dots, x_r \}$ of real-valued variables and the following system of equations over $V$:
	\begin{equation*}
		\Phi := 
		\begin{cases}
			a_{1,0} + a_{1,1} \cdot x_1 + \ldots + a_{1,r} \cdot x_r \geq  0\\
			\hfil \vdots\\
			a_{m,0} + a_{m,1} \cdot x_1 + \ldots + a_{m,r} \cdot x_r \geq 0\\
		\end{cases}.
	\end{equation*}
	Let $g_i$ be the LHS of the $i$-th inequality. If $\Phi$ is satisfiable, $\sat(\Phi)$ is compact, and $\Phi$ entails a polynomial inequality $g(x_1,\dots,x_r) > 0,$ then there exist non-negative real numbers $y_1,\dots y_u$ and polynomials $h_1,\dots,h_u \in \monoid(\Phi)$ such that:
	$$
	\textstyle g = \sum_{i=1}^u y_i \cdot h_i
	$$
	where $\monoid(\Phi) =  \left\{ \prod_{i=1}^m g_i^{k_i} \mid m,k_i \in \mathbb{N}\right\}$ is the semi-group of expressions in $\Phi$.
\end{theorem}

Handelman’s theorem, extends Farkas’ lemma by providing a characterization of the non-negativity of a polynomial over a set of linear inequalities. In such cases, given a technical parameter $d$, we first construct 
$\monoid_d(\Phi)~=~\left\{ \prod_{i=1}^m g_i^{k_i} \mid m,k_i \in \mathbb{N} \wedge \sum k_i \leq d\right\}$,
then introduce fresh variables $y_1, \dots y_{t}$, where $t=|\monoid_d(\Phi)|$, and convert (\ref{eq:ent}) into the following formula:
\[
\exists y_1, \dots \exists y_{t}. \bigwedge y_i \geq 0 \wedge \big[ g = \sum_{h_i \in \monoid_d(\Phi)} y_i \cdot h_i\big]
\]
The last equality represents a monomial-by-monomial equality over the polynomials $g$ and $\sum_{h_i \in \monoid_d(\Phi)} y_i \cdot h_i$. 

Putinar’s Positivstellensatz, extends both Farkas’ lemma and Handelman's Theorem by providing a characterization of the non-negativity of a polynomial over a set of polynomial inequalities.

\begin{theorem}[Putinar's Positivstellensatz \cite{putinar1993positive}]\label{theorem_put_pos}
	\index{Putinar's positivstellensatz}
	Given a finite collection of polynomials $\{g,g_1,\dots,g_k \} \in \mathbb{R}[x_1,\dots,x_n]$, let $\Phi$ be the set of inequalities defined as
	$$
	\Phi: \{g_1 \geq 0,  \dots , g_k \geq 0 \}.
	$$
	If $\Phi$ entails the polynomial inequality $\psi := g > 0$ and there exist some $i$ such that $\sat(g_i \geq 0)$ is compact, then there exist polynomials $h_0, \dots, h_k \in \mathbb{R}[x_1,\dots,x_n]$ such that 
	$$
	\textstyle g = h_0 + \sum_{i=1}^{m} h_i \cdot g_i 
	$$
	and every $h_i$ is a sum of squares (SOS). %Moreover, $\Phi$ is unsatisfiable if and only if $-1 > 0$ can be obtained as above, i.e.~with $g = -1$.
\end{theorem}

Similar to how we utilize Farkas' Lemma, we introduce fresh $h_i$ polynomials (with unknown coefficients) and add constraints on their coefficients to ensure they are SOS by applying \cite[Theorem 3.39]{blekherman2012semidefinite}. More details can be found in the appendix and in \cite{DBLP:conf/pldi/AsadiC0GM21}.

%\begin{compactitem}
%	\item \textbf{Farkas' Lemma.} This 
%	\item \textbf{Positivstellens\"atze Theorems.} These provide sound and semi-complete methods when either $\Phi$ or $\phi$ is non-linear.
%\end{compactitem}
Due to space restrictions, here we omit the details of how different types of inequalities are handled in the mentioned theorems and refer the reader to the Appendix for details.

